Measurements of the position-dependent photo-detection sensitivity of the Hamamatsu R11410 and R8520 photomultiplier tubes

The Hamamatsu R11410 and R8520 photomultiplier tubes (PMTs) are designed for applications in dark matter detectors using liquid xenon, featuring excellent sensitivity to VUV light and stable operability at cryogenic temperatures. For eleven R11410 and seven R8520 PMTs, we measured the relative photo-detection sensitivity at 470nm as a function of the position of the incident light on the photocathode. Considering 80% of the photocathode surfaces, the observed non-uniformity values are in the ranges of (5-10)% and (25-30)% for the R11410 and R8520 models, respectively. We found that the non-uniformity in the inner region of the photocathode surface is dominated by light reflections on the internal components of the photosensors and that the border regions contribute dominantly to the observed non-uniformity.

==> abstract <==
The XENON1T experiment, which is currently under construction
at the Laboratori Nationali del Gran Sasso (LNGS), is designed for direct detection of particle dark matter via scattering off xenon nuclei in a low-background, ultra-sensitive detector. It consists of a dual-phase time-projection chamber (TPC)
with 3 tons of liquid xenon, and 248 Hamamatsu R11410-21 photomultipliers (PMTs) which detect the primary scintillation light and electroluminescence signal. The intensity of the light is proportional to the amount of ionization charge released in a particle interaction with the target material. In order to have a deep
understanding of the experimental set-up, it is crucial to characterize the PMTs. Measurements of gain, resolution on single photoelectron spectrum,
linearity of the response and photocathode uniformity are therefore fundamental. 

For the
characterization of these PMTs a testing facility has been constructed,
in particular to measure photocathode uniformity.  This facility
provides a dark environment for the PMTs being tested, and includes hardware that allows
to perform the measurement fully automatically.

In this work I present how this new facility (\SandBox) for the detailed characterization of the XENON photosensors has been developed and
realized, successfully fulfilling the purpose to measure with high precision
(0.35 mm spatial resolution) the photocathode uniformity of different types of
PMTs. Each component is described in detail before presenting SandBox in its
complete and final configuration.  The measurement of the photocathode
uniformity has been performed using XENON1T PMTs.

In Chapter~\ref{chap:intro} the working principle and important properties of a
PMT are explained. Chapter~\ref{chap:blackbox} describes the design and the
features of the \SandBox{} measurement facility and in
Chapter~\ref{chap:measurement} the correct operation of SandBox is reported by
presenting measurements of the cathode uniformity for PMTs that will be used in
XENON1T.

